Directional Smoothness and Gradient Methods: Convergence and Adaptivity

We develop new sub-optimality bounds for gradient descent (GD) that depend on the conditioning of the objective along the path of optimization rather than on global, worst-case constants. Key to our proofs is directional smoothness, a measure of gradient variation that we use to develop upper-bounds on the objective. Minimizing these upper-bounds requires solving implicit equations to obtain a sequence of strongly adapted step-sizes; we show that these equations are straightforward to solve for convex quadratics and lead to new guarantees for two classical step-sizes. For general functions, we prove that the Polyak step-size and normalized GD obtain fast, path-dependent rates despite using no knowledge of the directional smoothness. Experiments on logistic regression show our convergence guarantees are tighter than the classical theory based on $L$-smoothness.

==> appendices/path_dependent_rates_proofs_c.tex <==
%!TEX root=../icml_dir_smooth.tex

\begin{restatable}{lemma}{directionalSC}\label{lemma:directional-sc}
    If \( f \) is convex, then for any \( y, x \in \R^d \),
    \begin{equation}
        f(y) \geq f(x) + \abr{\grad(x), y - x} + \frac{\mu(y, x)}{2}\norm{y - x}_2^2.
    \end{equation}
    If \( f \) is \( \mu \) strongly convex, then \( \mu(y, x) \geq \mu \).
\end{restatable}
\begin{proof}
    The fundamental theorem of calculus implies
    \begin{align*}
        f(x) - \abr{\grad(x), y - x}
         & = \int_{0}^1 \abr{\grad(x + t(y - x)) - \grad(x), y - x} dt \\
         & \geq \int_{0}^1 \mu(x, y) t \norm{x - y}_2^2 dt             \\
         & = \frac{\mu(x, y)}{2} \norm{y - x}^2_2.
    \end{align*}
    Note that we have implicitly used convexity to verify the inequality in the
    second line in the case where \( \mu(y, x) = 0 \).
    Now assume that \( f \) is \( \mu \) strongly convex.
    As a standard consequence of strong-convexity, we obtain:
    \begin{align*}
        \frac{\abr{\grad(x + t(y - x)) - \grad(x), y - x} }
        {t\norm{x-y}_2^2}
         & =\frac{\abr{\grad(x + t(y - x)) - \grad(x), x + t (y - x) - x} }
        {t^2 \norm{x-y}_2^2}                                                  \\
         & \geq \mu \frac{\norm{x - t(y - x) - x}_2^2}{t^2 \norm{y - x}_2^2}    \\
         & = \mu.
    \end{align*}
\end{proof}

\scSplitAnalysis*
\begin{proof}
    First note that \( \lambda_i < 0 \) for \( i \in \calG \) and \( \lambda_i
    \geq 0 \) for \( i \in \calB \).
    We start from \cref{eq:local-descent-lemma},
    \begin{align*}
        f(\xkk)
         & \leq f(\xk) + \etak\rbr{\frac{\etak M(\xkk, \xk)}{2} - 1}\norm{\grad(\xk)}_2^2                   \\
         & = f(\xk)
        + \mathbbm{1}_{k \in \calG} \cdot \sbr{\frac{\etak\lambda_k}{2} \norm{\grad(\xk)}_2^2 }
        + \mathbbm{1}_{k \in \calB} \cdot \sbr{\frac{\etak\lambda_k}{2} \norm{\grad(\xk)}_2^2}              \\
         & \leq f(\xk) + \mathbbm{1}_{k \in \calG} \cdot \sbr{\etak\lambda_k \mu_k \rbr{f(\xk) - f(\xopt)}}
        + \mathbbm{1}_{k \in \calB} \cdot \sbr{\frac{\etak\lambda_k}{2} \norm{\grad(\xk)}_2^2},
    \end{align*}
    where we used that directional strong convexity gives
    \[ \norm{\grad(\xk)}_2^2 \geq  2\mu_k \rbr{f(\xk) - f(\xopt)}. \]
    Subtracting \( f(\xopt) \) from both sides and then recursively applying the
    inequality gives the result.
\end{proof}

\scIteratesAnalysis*
\begin{proof}
    Let \( \Delta_k = \norm{\xk - \xopt}_2^2 \) and observe \[ \Delta_k =
        \norm{\xk - \xkk + \xkk - \xopt}_2^2 = \Delta_{k+1} + \norm{\xk - \xkk}_2^2 +
        2\abr{\xk - \xkk, \xkk - \xopt}.
    \]
    Using this expansion in \( \Delta_{k+1} - \Delta_k \), we obtain
    \begin{align*}
        \Delta_{k+1} - \Delta_k
         & = -\norm{\xk - \xkk}_2^2
        -2 \abr{\xk - \xkk, \xkk - \xopt}                                                 \\
         & = - \etak^2 \norm{\grad(\xk)}_2^2
        - 2 \etak \abr{\grad(\xk), \xkk - \xopt}                                          \\
         & = - \etak^2 \norm{\grad(\xk)}_2^2
        - 2 \etak \abr{\grad(\xk), \xkk - \xk}
        - 2 \etak \abr{\grad(\xk), \xk - \xopt}.
        \intertext{%
            Now we control the inner-products with directional strong convexity and
            directional smoothness.
        }
         & \leq - \etak^2 \norm{\grad(\xk)}_2^2
        - 2 \etak \abr{\grad(\xk), \xkk - \xk}
        + 2 \etak \sbr{f(\xopt) - f(\xk) - \frac{\mu_k}{2}\Delta_k}                       \\
         & \leq - \etak^2 \norm{\grad(\xk)}_2^2
        + 2 \etak \sbr{f(\xk) - f(\xkk) + \frac{M(\xkk, \xk)\etak^2}{2}\norm{\grad(\xk)}} \\
         & \qquad + 2 \etak \sbr{f(\xopt) - f(\xk) - \frac{\mu_k}{2}\Delta_k}             \\
         & = \etak^2\rbr{M(\xkk, \xk) \etak - 1} \norm{\grad(\xk)}_2^2
        + 2 \etak \sbr{f(\xopt) - f(\xkk)} - \mu_k \etak \Delta_k                         \\
         & \leq \etak^2\rbr{M(\xkk, \xk) \etak - 1} \norm{\grad(\xk)}_2^2
        - \mu_k \etak \Delta_k.
    \end{align*}
    Re-arranging this expression allows us to deduce a rate with
    error terms depending on the local smoothness,
    \begin{align*}
        \implies \Delta_{k+1}
         & \leq \rbr{1 - \mu_k \etak} \Delta_k
        + \etak^2\rbr{M(\xkk, \xk) \eta - 1} \norm{\grad(\xk)}_2^2  \\
         & \leq \sbr{\prod_{i=0}^k \rbr{1 - \mu_i \eta_i}} \Delta_0
        + \sum_{i=0}^k \sbr{\prod_{j = i+1}^k \rbr{1 - \mu_j \eta_j}}
        \eta_i^2 \rbr{M(\x_{i+1}, \x_i) \eta_i - 1} \norm{\grad(\x_i)}_2^2.
    \end{align*}
\end{proof}

\convexAnyStepsize*
\begin{proof}
    Let \( \Delta_k = \norm{\xk - \xopt}_2^2 \) and observe \[ \Delta_k =
        \norm{\xk - \xkk + \xkk - \xopt}_2^2 = \Delta_{k+1} + \norm{\xk - \xkk}_2^2 +
        2\abr{\xk - \xkk, \xkk - \xopt}.
    \]
    Using this expansion in \( \Delta_{k+1} - \Delta_k \), we obtain
    \begin{align*}
        \Delta_{k+1} - \Delta_k
         & = -\norm{\xk - \xkk}_2^2
        -2 \abr{\xk - \xkk, \xkk - \xopt}                                                             \\
         & = - \etak^2 \norm{\grad(\xk)}_2^2
        - 2 \etak \abr{\grad(\xk), \xkk - \xopt}                                                      \\
         & = - \etak^2 \norm{\grad(\xk)}_2^2
        - 2 \etak \abr{\grad(\xk), \xkk - \xk}
        - 2 \etak \abr{\grad(\xk), \xk - \xopt}.
        \intertext{
            Now we use convexity and directional smoothness to control
            the two inner-products as follows:
        }
        \Delta_{k+1} - \Delta_k
         & \leq - \etak^2 \norm{\grad(\xk)}_2^2
        - 2 \etak \rbr{f(\xk) - f(\xopt)}
        - 2 \etak \abr{\grad(\xk), \xkk - \xk}                                                        \\
         & \leq - \etak^2 \norm{\grad(\xk)}_2^2
        - 2 \etak \rbr{f(\xk) - f(\xopt)}
        + 2 \etak (f(\xk) - f(\xkk))
        + \etak^3 M(\xkk, \xk) \norm{\grad(\xk)}_2^2                                                  \\
         & = \etak^2 (\etak M(\xkk, \xk) - 1)\norm{\grad(\xk)}_2^2 - 2\etak \rbr{f(\xkk) - f(\xopt)}.
    \end{align*}
    Re-arranging this equation and summing over iterations implies the following
    sub-optimality bound:
    \begin{align*}
        \sum_{i=0}^k \frac{\eta_{i}}{\sum_{i=0}^k \eta_i} \rbr{f(x_{i+1}) - f(\xopt)}
         & \leq \frac{\Delta_{0} + \sum_{i=0}^{k} \eta_i^2 (\eta_i M(\x_{i+1}, \x_i) - 1)\norm{\grad(\x_i)}_2^2}{2\sum_{i=0}^k \eta_i}.
        \intertext{Convexity of \( f \) and Jensen's inequality now imply the final result,}
        \implies
        f(\bar x_k) - f(\xopt)
         & \leq \frac{\Delta_{0} + \sum_{i=0}^{k} \eta_i^2 (\eta_i M(\x_{i+1}, \x_i) - 1)\norm{\grad(\x_i)}_2^2}{2\sum_{i=0}^k \eta_i}.
    \end{align*}
\end{proof}



==> sections/path_dependent_rates_c.tex <==
%!TEX root=../icml_dir_smooth.tex

\begin{figure*}[t]
    \centering
    \input{figures/quadratic_bound}
    \caption{Illustration of GD with \( \etak = 1 / L \).
        Even though the step-size exactly minimizes the upper-bound from \( L
        \)-smoothness, \( M_i \) directional smoothness better predicts the progress
        of the gradient step.
        Our rates improve on \( L \)-smoothness because of this tighter bound.
    }
    \label{fig:quadratic-bound}
\end{figure*}

Given directional smoothness $M$, we obtain a version of the
descent lemma which depends only on local geometry,
\begin{equation}
    \label{eq:local-descent-lemma}
    f_{k+1} \leq f_k -
    \rbr{\etak - \frac{\etak^2 M(\xkk, \xk)}{2}} \norm{\grad(\xk)}_2^2,
\end{equation}
where \( f_{k} = f(\xk) \) and \( f_{k+1} = f(\xkk) \)
(see \Cref{lemma:local-descent-lemma}).
If \( \etak < 2 / M(\xkk, \xk) \), then GD is guaranteed to decrease the
function value and we call \( \etak \) \emph{adapted} to $M(\xkk, \xk)$.
However, finding a sequence of adapted step-sizes is not always
straightforward.
For instance, computing \( \etak = 1 / M(\xkk(\etak), \xk) \) requires solving
a non-linear equation.

%% Rob: This comment here at this stage is a bit confusing. It doesn't matter now that it's analogous to 1/L
%the standard \( 1 / L \) analogue requires solving the
%non-linear equation \( \etak = 1 / M(\xkk(\etak), \xk) \) which is non-trivial.
%We discuss how to compute adapted step-sizes in \Cref{sec:adapt-learn-rates}.

The rest of this section leverages directional smoothness to derive new
guarantees for GD with arbitrary step-sizes.
We emphasize that the following results are \emph{sub-optimality bounds},
rather than convergence rates; a sequence of adapted step-sizes is required to
convert our propositions into a convergence theory.
As a trade-off, we obtain bounds reflecting the locality of GD, rather than
treating it as a global method.

We start with the case when \( f \) has lower curvature.
Instead of using strong convexity or the PL-condition \citep{karimi2016linear},
we propose the directional strong convexity constant,
\begin{equation}
    \label{eq:directional-sc-constant}
    \mu(y, x)
    \!=\! \inf_{t\in [0,1]} \frac{\abr{\grad(x \!+\! t(y \!-\! x)) \!-\! \grad(x), y \!-\! x} }
    {t\norm{y - x}_2^2}.
\end{equation}
If \( f \) is convex, then \( \mu(y, x) \) is non-negative and verifies the
standard lower-bound from strong convexity,
\begin{equation}
    \label{eq:directional-sc}
    f(y) \geq f(x) + \abr{\grad(x), y - x} + \frac{\mu(y, x)}{2}\norm{y - x}_2^2.
\end{equation}
Moreover, we have \( \mu(y, x) \geq \mu \) when \( f \) is $\mu$--strongly
convex.
We prove two bounds for convex functions using directional strong convexity.
For brevity, we denote \( M_i := M(\x_{i+1}, \x_i) \), \( \mu_i :=
\mu_i(\x_{i+1}, x_i) \), \( \delta_i = f(x_i) - f(\xopt) \), and \( \Delta_i =
\norm{x_i - \xopt}_2^2 \), where \( \xopt \) is a minimizer of \( f \).

\begin{restatable}{proposition}{scSplitAnalysis}\label{prop:sc-split-analysis}
    If \( f \) is convex with minimizer $\xopt$, then GD with step-size
    sequence \( \cbr{\etak} \) satisfies,
    \begin{equation}
        \label{eq:sc-split-analysis}
        \begin{split}
            \delta_{k+1}
             & \leq \sbr{\prod_{i \in \calG} \rbr{1 + \eta_i \lambda_i \mu_i}}
            \delta_0                                                                                  \\
             & + \sum_{i \in \calB} \sbr{\prod_{j > i, j \in \calG} \rbr{1 + \eta_j \lambda_j \mu_j}}
            \frac{\eta_i \lambda_i}{2} \norm{\grad(\x_i)}_2^2,
        \end{split}
    \end{equation}
    where \( \lambda_i \!=\! \eta_i M_i \!-\! 2 \),
    \( \calG = \cbr{i : \eta_i \!<\! \frac{2}{M(\x_{i+1}, \x_{i})}} \),
    \( \calB = [k] \!\setminus\! \calG \).
\end{restatable}
The analysis splits iterations into good steps $\mathcal{G}$, where \( \etak
\) is adapted to the directional smoothness, and bad steps $\calB$, where the
step-size is too large and GD may increase the optimality gap.
When \( f \) is \( L \)-smooth and \( \mu \)-strongly convex,
using the step-size sequence \( \etak = 1 / L \) gives
\begin{equation}
    \label{eq:sc-tighter-rate}
    \frac{f(\xkk) - f(\xopt)}{f(\x_0) - f(\xopt)}  \leq  \left[ \prod_{i = 0}^{k}
        \rbr{1 - \frac{\mu_i \rbr{2 - M_i / L}}{L}} \right]
\end{equation}
where \( \mu_i \rbr{2 - M_i / L} \geq \mu \).
As a result, \Cref{eq:sc-split-analysis} gives a at least as tight a rate
under standard assumptions by localizing to the convergence path as described
by \emph{any} directional smoothness $M$.
When \( M_k < L \), the gap in constants yields a strictly improved rate, as
shown by \cref{fig:quadratic-bound}.
We also prove the following, more elegant bound.

\begin{restatable}{proposition}{scIteratesAnalysis}\label{prop:sc-iterates-analysis}
    If $f$ is convex with minimizer $\xopt$, then GD with step-size
    sequence \(\cbr{\etak} \) satisfies,
    \begin{equation}
        \label{eq:sc-iterates-analysis-eq}
        \begin{split}
             & \Delta_{k+1}
            \leq \sbr{\prod_{i=0}^{k} \rbr{1 - \mu_i \eta_i}} \Delta_0                          \\
             & \hspace{1em} +\! \sum_{i=0}^k \sbr{\prod_{j > i} \rbr{1 \!-\! \mu_j \eta_j}}\!\!
            \rbr{M_i \eta_i^3 \!-\! \eta_i^2} \norm{\grad(\x_i)}_2^2.
        \end{split}
    \end{equation}
\end{restatable}
Unlike \Cref{prop:sc-split-analysis}, this analysis shows linear progress at
each iteration and does not divide \( k \) into good steps and bad steps.
In exchange, the second term in \Cref{eq:sc-iterates-analysis-eq} reflects how
much convergence is degraded when \( \etak \) is not adapted to the
directional smoothness function $M$.
% Moreover, since
% local smoothness only affects the step-size, choosing a fixed step-size
% does not reveal the same path-dependence.

We conclude this section with a bound for when there is no lower curvature,
meaning \( \mu_i = 0 \).
\begin{restatable}{proposition}{convexAnyStepsize}\label{prop:convex-any-stepsize}
    Let \( \bar x_k = \sum_{i=0}^k \eta_i x_{i+1} / \sum_{i=0}^k \eta_i \).
    If \( f \) is convex with minimizer $\xopt$, then GD satisfies,
    \begin{equation}
        \label{eq:1}
        \begin{split}
            f(\bar x_k) - f(\xopt)
             & \leq \frac{\norm{x_0 - \xopt}_2^2}{2\sum_{i=0}^k \eta_i}                                       \\
             & + \frac{\sum_{i=0}^{k} \eta_i^2 (\eta_i M_i - 1)\norm{\grad(\x_i)}_2^2}{2\sum_{i=0}^k \eta_i}.
        \end{split}
    \end{equation}
\end{restatable}

% Specializing this rate with to \( \etak = 1 / L \) and \( M_i = A_i < L \) shows,
% \begin{equation}
%    f(\bar x_k) - f(\xopt)
%    \leq \frac{L \norm{x_0 - \xopt}_2^2 + \sum_{i=0}^{k} (A_i / L - 1)\norm{\grad(\x_i)}_2^2 / L}{2 K}.
% \end{equation}
This rate is at least as tight as the standard analysis because $M_i \leq L.
$
It is key to our developments in the next sections.
%This rate, which is at least as tight as the standard analysis, is key
%to our results in the next sections.
% \Cref{prop:convex-any-stepsize} with \( \etak = 1 / L \) and
% \( M_i = A_i \) gives a rate which adapts to the optimization path
% and is at least as fast as the standard analysis.

